Out-of-distribution Prediction with Invariant Risk Minimization: The Limitation and An Effective Fix

This work considers the out-of-distribution (OOD) prediction problem where (1)~the training data are from multiple domains and (2)~the test domain is unseen in the training. DNNs fail in OOD prediction because they are prone to pick up spurious correlations. Recently, Invariant Risk Minimization (IRM) is proposed to address this issue. Its effectiveness has been demonstrated in the colored MNIST experiment. Nevertheless, we find that the performance of IRM can be dramatically degraded under \emph{strong $\Lambda$ spuriousness} -- when the spurious correlation between the spurious features and the class label is strong due to the strong causal influence of their common cause, the domain label, on both of them (see Fig. 1). In this work, we try to answer the questions: why does IRM fail in the aforementioned setting? Why does IRM work for the original colored MNIST dataset? How can we fix this problem of IRM? Then, we propose a simple and effective approach to fix the problem of IRM. We combine IRM with conditional distribution matching to avoid a specific type of spurious correlation under strong $\Lambda$ spuriousness. Empirically, we design a series of semi synthetic datasets -- the colored MNIST plus, which exposes the problems of IRM and demonstrates the efficacy of the proposed method.

==> exp_backup.tex <==
\subsection{Verifying the Non-overlapping Problem with Colored MNIST}

Here, we empirically verify the conjecture that deep neural network models suffer from the non-overlapping problem when they are trained by loss functions regularized by the IRMv1 penalty term (Eq.~\ref{eq:IRMv1}).
%

Here, we train MLP and LeNet-5 models on the Colored MNIST dataset~\citep{arjovsky2019invariant} to examine the existence of non-overlapping problem of the IRMv1 regularized models when the model becomes deep or overparameterized.
%
First, we use the widely adopted T-SNE technique~\citep{maaten2008visualizing} to plot the representations learned by the first layer and the second last layer and show to what degree data points from different environments are non-overlapping.
%
Second, given instances from the first and the third environments, we examine the accuracy of binary classifiers in the task of predicting the environment label of each instance in the representation space.
%
Intuitively, more accurate the classifiers are, the more likely the representations embed the environment label (i.e., the overlapping is worse).
%
% Third, after training the neural networks, we train a two-layer MLP to predict environment labels.
%
% Then we extract its intermediate outputs to examine whether the non-overlapping problem exists.

\noindent\textbf{T-SNE Plots.}
%
\begin{figure}[tb]
\centering
\begin{minipage}{0.32\textwidth}
\centering
\subfigure[MLP trained by ERM]
{\label{fig:MLP_ERM}\includegraphics[width=\textwidth]{figs/MLP_ERM.png}}
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\subfigure[MLP trained by IRM]
{\label{fig:MLP_IRM}\includegraphics[width=\textwidth]{figs/MLP_IRM.png}}
\end{minipage}
\hfil
\begin{minipage}{0.32\textwidth}
\centering
\subfigure[Oracle MLP]
{\label{fig:MLP_Oracle}\includegraphics[width=\textwidth]{figs/MLP_Oracle.png}}
\end{minipage}
\caption{T-SNE plots of representations learned by MLP models trained with ERM and IRM, and the oracle grayscale MLP model.}
\label{fig:TSNE_MLP}
\end{figure}
%
Fig.~\ref{fig:TSNE_MLP} shows the T-SNE plots of the representations learned by three MLP models on the Colored MNIST dataset.
%
We can observe that in Fig.~\ref{fig:MLP_ERM} and~\ref{fig:MLP_IRM}, in the representation space learned by the ERM and IRM models, the test instances from the third environment (blue dots) are more likely to appear in certain regions. This implies that these two models utilize the environment label to minimize the negative log likelihood on the training set.
%
While as Fig.~\ref{fig:MLP_Oracle} shows, the oracle MLP model does not suffer from the non-overlapping problem.
%
This is because the oracle MLP model only takes causal features as its input.
%
Thus, it cannot leverage the environment variable to minimize the negative log likelihood in training phase.

\noindent\textbf{Classification Results.}
To further verify the observations from the T-SNE plots, we report the classification results in the representation spaces learned by the LeNet-5 models.
%

\subsection{Which Layers Does the IRMv1 Help?}

Understanding which layer suffers the most from the non-overlapping problem has important implication on the design of methods to mitigate this problem.
%
Here, given the representations learned by the first Convolutional layer and the second last fully connected layer of a LeNet-5 architecture, we examine the degree of non-overlapping environment classification results with logisitic regression, SVM and random forest.
%


% \subsection{How does Non-overlapping Happen?}
% Now, we conjecture that non-overlapping happens when the model overfits to the IRMv1 regularization term.
% %
% This is based on the observation that test accuracy surges to the oracle level right after the IRMv1 penalty term is plugged in but then converges to around $0.5$.

% \subsection{Can the Non-overlapping Problem Be Mitigated?}





% Here, we use TSNE plots along with two metrics to measure whether there exists the non-overlapping problem.
%
% Specifically, we apply these techniques to analyze the representations that are the outputs of the second last layer of a neural network (e.g., a MLP or a LeNet-5).
%

% \noindent\textbf{Computing the Pairwise Distance.}
%
% Pairs of instances are uniformly randomly sampled from the whole dataset. Each pair $(i,j)$ belongs to one the six groups: $e_i=e_j=1$, $e_i=e_j=2$, $e_i=e_j=3$, $e_i=1,e_j=2$, $e_i=1,e_j=3$, and $e_i=2, e_j=3$. Then we calculate the average pairwise squared Euclidean distance for each group and observe how they change with the number of training iterations.
%


\subsection{Results on Colored MNIST}

Here, we split the training data into 20,000 training and 5,000 validation for each training environment.
%
We select the model with the least validation loss after the penalty terms are added.
%
We run each method with batch size 5,000 for 1,000 steps.
%
We report the experimental results in Table~\ref{tab:cmnist_results}.
%


==> intro.tex <==
\section{Introduction}

Empirical results have shown the efficacy of deep learning algorithms in a variety of areas including computer vision, natural language processing and speech recognition.
%
However, such positive results overwhelmingly rely on the assumption that the underlying distributions of the training, validation and test data are very similar if not the same.
%
In other words, out-of-distribution (OOD) generalization beyond the training data still remains a challenging problem for deep neural networks (DNNs).
% In this work, we focus on the problem of OOD generalization where the training data are collected from multiple domains which are dramatically different from the domain of test data.
%


The transportability of causal relationships~\citep{pearl2011transportability} across domains turns out to be the key to address the OOD generalization problem.
%
While spurious correlations learned in one domain are often untenable in another, the transportability of causal relationships enables DNNs to generalize to unseen domains.
%
Without knowing the underlying causal graph, a general recipe for DNNs to capture causal relationships is to learn causal feature representations which hold invariant causal relationships with the label.
%
Thus, the main challenge of OOD generalization is to learn causal feature representations given only observational training data. 

%
Recently, Invariant Risk Minimization (IRM)~\citep{arjovsky2019invariant} is proposed to address the problem.
%
IRM is initially formulated as a constraint: the learned feature representation must

\begin{figure}[tbh!]
    \centering
    \begin{tikzpicture}
\centering
    % x node set with absolute coordinates
    \node[state] (e) at (-2,0) {$E$};
    \node[state] (xc) at (0,0) {${X}^c$};

    % y node set relative to x.
    % Locations can be:
    % right,left,above,below,
    % above left,below right, etc
    \node[state] (y) at (2,0) {$Y$};
    % \node[state,dashed] (h) at (-2,1) {$\mathbf{h}$}; 
    \node[state] (xs) at (0,1) {${X}^s$}; 

    % Directed edge
    \path (e) edge (xc);
    \path (e) edge (xs);
    \path (xc) edge (y);
    % \path (h) edge (a);
    % \path (t) edge (y);
    % Bidirected edge
    % \path[bidirected] (x) edge[bend left=60] (y);
\end{tikzpicture}
    \caption{The causal diagram representing the out-of-distribution generalization problem.
    %
    The influence of domain variable $E$ on the label $Y$ is mediated by the causal features ${X}^c$.
    %
    With different values of $E$, feature distributions $P({X}^s|E)$ and $P({X}^c|E)$ may change.
    %
    But the predictive distribution with causal features $P(Y|{X}^c)$ remains the same.
    %
    The directed edges are causal relationships. %
    % The solid circles represent observed variables.
    % and the dashed circle stands for hidden confounders.}
    }
    \label{fig:causal_graph1}
\end{figure}

We consider a prediction problem with observed instances $\{{x}_i^e,y_i^e\}_{i=1}^{N^e},e=1,...,|\mathcal{E}|$ from a set of environments $\mathcal{E}$.
%
The feature distributions $P(X^s|E)$ and $P(X^c)$ can vary by environments. 
%
Only instances from a subset of the environments, $\mathcal{E}_{tr} \subset \mathcal{E}$, are available in the training phase.
%
Deep neural networks often can be formulated as two functions: a representation learning function $g:\mathcal{X}\rightarrow\mathds{R}^d$ and a label prediction function $f:\mathds{R}^d\rightarrow\mathcal{Y}$.
%
For learning deep neural networks for out-of-distribution generalization, Arjovsky et al.~\citep{arjovsky2019invariant} propose a heuristic inductive bias as a regularizer, Invariant Risk Minimizaton (IRM). IRM conjectures that feature representations $g({x}_i)$ that can achieve optimal prediction functions $f^*$ across all training environments $\mathcal{E}_{tr}$ are able to generalize to out-of-distribution predictions to those $\mathcal{E}\setminus\mathcal{E}_{tr}$.
%

Given the representation function $g$, suppose we have two different label prediction functions $f$ and $f^e$, where $f^e$ takes the environment variable as its input along with the representations.
%
Ideally, we hope $f(g({x}))$ would be quite similar to $f^e(g({x}),e)$ if they are not the same.

\textbf{The Non-overlapping Problem.} IRM confronts the problem of non-overlapping in the feature representation space.
%
In an extreme case, this happens when the representation learning function satisfies $g({x}|e)\not = g({x}'|e'), e\not = e', \forall ({x}, {x}')$.
%
In this situation, obtaining the optimal prediction functions $f^*$ in different environments become orthogonal tasks, which means achieving them simultaneously becomes trivial. Therefore, the IRM regularization term would have no effect for learning invariant feature.
%
From another perspective, even if a model is not utilizing the environment variable $E$ as a feature to predict the label $Y$, the environment variable is implicitly utilized by the discriminative model $f$ due to the differences in the representation distributions $D(P(g({x})|e)||P(g({x}|e')))$.
%
Approaches based on Generative Adversarial Networks~\citep{goodfellow2014generative} can be developed to obtain balanced distributions of representations.
%
However, when the discriminator is too strong, this approach can be problematic.
%
A too strong discriminator means the error backpropagated by it may have very limited contribution toward the goal of representation balancing.
%

An alternative approach to this is to directly minimize the divergences between the representation distributions.
%
Divergence metrics can be challenging to compute in the high-dimensional representation space.
%
In~\citep{kingma2013auto}, the reparameterization trick is proposed to allow applying backpropagation and SGD for maximizing the ELBO~\citep{blei2017variational} of a regularized log likelihood of observed instances with deep latent-variable models.
%
Tolstikhin et al.~\citep{tolstikhin2017wasserstein} extend this work.
%
They find that VAE minimizes the KL divergence between the approximate posterior $Q(Z|X)$ and the prior $P(Z)$, which can be problematic as the conditional $Q(Z|X)$ is only evaluated at the observed instances while the prior $P(Z)$ is the exact probability density.
%
To overcome this problem, they aim to minimize the divergence between the continuous approximated marginal distribution $Q({Z}) = \int Q({Z}|{X})P({X})d{X}$ and the prior $P({Z})$.
%







% \noindent\textbf{out-of-distribution Generalization in Face Verification Problem.}
% In this problem, given a pair of test images, the task is to determine whether the two images are photos of the same individual.
% % A false positive means an image of an unenrolled individual is matched to an image in the database.
% %
% In this problem, the environment variable (e.g., poses) is a cause of the label.
% %
% We adapt the causal graph provided by the challenge\footnote{\url{http://chalearnlap.cvc.uab.es/challenge/38/description/}}, to describe this problem as Fig.~\ref{fig:causal_graph2}.

% \begin{figure}[tbh!]
%     \centering
%     \begin{tikzpicture}
% \centering
%     % x node set with absolute coordinates
%     \node[state] (e) at (-2,0) {$E$};
%     \node[state] (xc) at (0,0) {$\bm{X}^c$};

%     % y node set relative to x.
%     % Locations can be:
%     % right,left,above,below,
%     % above left,below right, etc
%     \node[state] (y) at (2,0) {$Y$};
%     % \node[state,dashed] (h) at (-2,1) {$\mathbf{h}$}; 
%     \node[state] (xs) at (0,1) {$\bm{X}^s$}; 

%     % Directed edge
%     \path (e) edge (xc);
%     \path (e) edge (xs);
%     \path (xc) edge (y);
%     % \path (h) edge (a);
%     % \path (t) edge (y);
%     % Bidirected edge
%     % \path[bidirected] (x) edge[bend left=60] (y);
%      \path (e) edge[bend left=-30] (y);
% \end{tikzpicture}
%     \caption{The causal diagram representing the face verification problem.
%     %
%     The influence of environment variable $E$ on the label $Y$ is direct and also mediated by causal features $\bm{X}^c$.
%     %
%     This implies we may need to model $P(Y|E)$ to control the influence of the environment $E$ on the label $Y$.
%     %
%     By excluding such influence, the invariant causal relationship from $\bm{X}^c$ to $Y$ can be captured. 
%     %
%     % With those unseen environments $e'\in\mathcal{E}\setminus\mathcal{E}_{tr}$, we may use $P(Y|\bm{X})$ to approximate $P(Y| E)$. %
%     %
%     If we assume that we are able to learn representations $h(\bm{x})$ of features that are predictive of the environment.
%     %
%     Then, when we consider an environment $e'$ that only appears in the test set, we can make use of the representations $h(\bm{x})$ that are used to model $P(E|h(\bm{x}))$. This is because $h(\bm{x})$ catches the pattern of the new environment $e'$, which allows us to control the influence of the environment variable on the label for out-of-distribution prediction.  
%     % When the value of $E$ changes, feature distributions $P(\bm{X}_s|E)$ and $P(\bm{X}_c|E)$ can change.
%     %
%     % However, the predictive distribution with causal features $P(Y|\bm{X}_c)$ remains the same.
%     %
%     The directed edges signify causal relations. The solid circles represent observed variables.
%     % and the dashed circle stands for hidden confounders.}
%     }
%     \label{fig:causal_graph2}
% \end{figure}
% For example, if the label of an image is positive, the necessary condition is that the environment variable takes a the value corresponding to the 


==> method.tex <==
\section{Methodology}

\subsection{Assumptions of Existing Invariant Representation Learning Methods.}

\begin{itemize}
    \item IRM~\citep{arjovsky2019invariant}: $Y\independent E|\Phi(\bm{X})$. A variant is to measure variance directly with environment-specific risks $R^{e}(\phi)=\mathcal{L}^{e}\left(f_{-e} \circ \Phi(\bm{X})\right)-\mathcal{L}^{e}\left(f_{e} \circ \Phi(\bm{X})\right)$~\citep{jin2020domain}.
    
    \item Domain Adaptation: $P(\Phi(\bm{X})|e) = P(\Phi(\bm{X})|e')$
    
    \item Conditional Domain Adaptation: $P(\Phi(\bm{X})|y,e) = P(\Phi(\bm{X})|y,e')$
    
    \item Robust Optimization~\citep{ben2009robust}: 
    % Minimizing the worst environment risk $\mathcal{R}_{\mathrm{RI}}(\theta) \doteq \max _{\Sigma_{e} \lambda_{e}=1 \atop \lambda_{e} \geq 0} \sum_{e} \lambda_{e} \mathcal{R}_{e}(\theta)$.
    The underlying assumption is $R^e(\Phi(\bm{X}))=R^{e'}(\Phi(\bm{X}))$.
    \cite{sagawa2019distributionally} show that strong regularization (e.g., early stopping and strong $L_2$ regularization) is needed for over-parameterized models.
    
    % \item Data Augmentation~\citep{ilse2020designing}. we are successfully augmenting all high-level features.
\end{itemize}

% Here, we propose a novel method to fix the non-overlapping problem of the IRM framework for fair face verification and recognition.
%
We first consider IRMV1 as a baseline loss function. It is a weighted sum of two loss functions.
\begin{equation}
\begin{split}
\mathcal{L} &= \mathcal{L}_{main} + \lambda \mathcal{L}_{IRM_{V1}}\\
    \mathcal{L}_{IRM_{V1}} &= \sum_{e\in\mathcal{E}_{tr}}||\bigtriangledown_{w|w=1.0}R^e(wg(\bm{x}),y)||_2^2 \\
    % \mathcal{L}_{Overlap} &= \sum_{e\in\mathcal{E}_{tr}} D(P(g(\bm{x})|e)||P(g(\bm{x}))),
    \label{eq:IRMv1}
\end{split}
\end{equation}
where $\mathcal{L}_{main}$ is the main loss function for the face verification problem (e.g., Focal loss~\citep{lin2017focal} and Triplet loss~\citep{schroff2015facenet}). 
%

\noindent\textbf{Solving the Non-overlapping Problem of IRM.}
%
To enforce the causal representations of different environments to be overlapped.
%
We can explicitly minimize the divergences between the conditional causal feature representation distributions and the corresponding marginal distribution:
\begin{equation}
   \mathcal{L}_{overlap} = \sum_{e\in\mathcal{E}_{tr}} D(P(g(\bm{x})|e)||P(g(\bm{x}))).
   \label{eq:overlap_loss}
\end{equation}

We know that computing the divergence between two high-dimensional distributions parameterized by deep neural networks can be extremely challenging~\citep{tolstikhin2017wasserstein}.
%
GAN-based approaches and estimators of divengences (the Wasserstein-1 distance estimator~\citep{cuturi2014fast}) can be adopted here to compute the divergences in Eq.~\ref{eq:overlap_loss}.
% We also need to consider those environments that are not observed in the training set.
%
% Maybe we can use a Determinantal Point Process (DPP) to sample diverse instances for fast computation of the loss in Eq.~\ref{eq:overlap_loss}.


\subsection{Proposed Methods.}
Here, we introduce the proposed variants of IRMv1.
%

\noindent\textbf{Model5.} Model5 describes the family of methods that compensate the IRMv1 loss with conditional distribution matching. Conditional distribution matching refers to the goal to minimize the divergence $D(P(F(X)|Y,E=e)||P(F(X)|Y,E=e')),e\not=e'$, or equivalently, $D(P(F(X)|Y)||P(F(X)|Y,E))$.

\noindent\textit{Balancing Logits.}
Motivated by the fact that IRMv1 and conditional distribution matching are two necessary conditions for learning invariant features (Eq.~\ref{def:invariant}), we propose to impose both necessary conditions simultaneously.
We formulate the loss function as:
\begin{equation}
    \mathcal{L}_{model5} = \mathcal{L}_{main} + \lambda_1 \mathcal{L}_{cdm} + \lambda_2 \mathcal{L}_{IRMv1},
    \label{eq:model5v1}
\end{equation}
The conditional distribution matching penalty $\mathcal{L}_{cdm}$ is estimated by the Jensen-Shannon divergence:
\begin{equation}
    \mathcal{L}_{cdmv1}= \frac{1}{2} \sum_{y=0,1} D_{JS}(P(\hat{Y}=1|Y=y,E=e)||P(\hat{Y}=1|Y=y,E=e'))),
\end{equation}
$\mathds{E}_{x\sim P(X|Y=y,E=e),x'\sim P(X|Y=y,E=e')}[D_{JS}(\sigma(F(x)),\sigma(F(x')))]$, $F(X)$ denotes the logits, and $\sigma(x)=\frac{1}{1+\exp(-x)}$ is the sigmoid function.
%



%
\noindent\textit{Conditional Distribution Matching with MMD.}
Minimizing this JS divergence balances the conditional distributions of logits $P(F(X)|Y,E)$ since the sigmoid function is an ingestive function.
%
However, this method cannot be directly applied to balance the distributions of representations from intermediate layers as $P(F(X)|Y,E)$ may not be easy to estimate. Not to mention the mini-batch estimation of JS divergence is biased.
%
Therefore, we adopt the Integral Probability Metrics (IPMs)~\citep{lopez2016revisiting}.
%

Given a class of functions $h:\mathcal{X}\rightarrow\mathds{R}$, an IPM between two distributions $P$ and $Q$ is defined as:
\begin{equation}
    \mathrm{IPM}(P,Q) = \sup_{h}(\mathds{E}_{x\sim P}[h(x)]-\mathds{E}_{x'\sim Q}[h(x')]).
\end{equation}
%
Maximum Mean Discrepancy (MMD) is one of the widely adopted IPMs~\citep{li2017mmd}.
%
IPM reduces to MMD when $h\in\{h':||h'||_{\mathcal{H}}\le 1\}$.
%
Here, we adopt the MMD metric with inverse multiquadratics (IMQ) kernel. The IMQ kernel is defined as $k(x,x')=C/(C+||x-x'||_2^2)$.
%
Let $P=P(F(X)|Y=y,E=e)$ and $Q=P(F(X)|Y=y,E=e')$ we calculate the squared MMD as:
\begin{equation}
\mathcal{L}_{cdm} = \sum_{y}\sum_{(e,e')}\mathrm{MMD}^{2}({P},{Q})=\sum_{y}\sum_{(e,e')}\left\|\mu_{P}-\mu_{Q}\right\|_{\mathcal{H}}^{2}=\left\langle\mu_{P}, \mu_{P}\right\rangle_{\mathcal{H}}+\left\langle\mu_{{Q}}, \mu_{{Q}}\right\rangle_{\mathcal{H}}-2\left\langle\mu_{{P}}, \mu_{{Q}}\right\rangle_{\mathcal{H}},
\label{eq:MMD}
\end{equation}
where $\mu_P = \mathds{E}_{x\sim P}[\phi(x)]$ and $\mu_Q = \mathds{E}_{x\sim Q}[\phi(x)]$ and $\phi:\mathcal{X}\rightarrow \mathcal{H}$ is a mapping s.t. its corresponding kernel $k(x,x') = \left\langle \phi(x),\phi(x')\right\rangle_{\mathcal{H}}$.
%
Each term on the RHS of Eq.~\ref{eq:MMD} can be computed by  \begin{equation}
\begin{split}
    \left\langle\mu_{{P}}, \mu_{{P}}\right\rangle_{\mathcal{H}} = \mathds{E}_{x\sim P, x' \sim P}[k(x,x')] = \frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n k(x_i,x_j') \\
        \left\langle\mu_{{Q}}, \mu_{{Q}}\right\rangle_{\mathcal{H}} = \mathds{E}_{x\sim Q, x' \sim Q}[k(x,x')] = \frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n k(x_i,x_j') \\
            \left\langle\mu_{{P}}, \mu_{{Q}}\right\rangle_{\mathcal{H}} = \mathds{E}_{x\sim P, x' \sim Q}[k(x,x')] = \frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n k(x_i,x_j')\\
    \end{split}
\end{equation}

\noindent\textit{Conditional Distribution Matching with GAN loss.}
%
Without knowing $P(F(X)|Y,E)$, another method is develop a minimax game to minimize the IPM between $P(F(X)|Y,E=e)$ and $P(F(X)|Y,E=e')$ or that between $P(F(X)|Y,E)$ and $P(F(X)|Y)$.
%
Let $\mathcal{F}$ denote the feature representation space, a discriminator $D^y:\mathcal{F}\rightarrow [0,1]$ is defined for each class $y$.
%
Thus, in the minimax game, we can train $F(X)$ and $D^y$ alternatively.
%
In particular, we train $F(X)$ to fool each discriminator $D^y$ by minimizing its log-likelihood and train each discriminator $D^y$ by maximizing its log-likelihood:
\begin{equation}
    \mathcal{L}_{cmd} = \sum_y
    % \underset{F}{\min}\underset{D^y}{\max}
    \max_{D^y}
    \; \sum_{e} \alpha_e^y \mathds{E}_{x\sim P(X|Y=y,E)}\log(D^y(F(x))) + \mathds{E}_{x'\sim P(X|Y)}\log(1-D^y(F(x'))),
    \label{eq:JS_GAN}
\end{equation}
where $\alpha_e^y =  P(E=e|Y=y)$ denotes the importance of environment $e$ among the instances from class $y$.
%
We can show this is equivalent to minimizing the JS divergence between $D_{JS}(P(F(X)|Y,E)||P(F(X)|Y))$.
%

Without considering the negative samples, we have the simplified conditional distribution matching loss as:
\begin{equation}
        \mathcal{L}_{cmd} = \sum_y
    % \underset{F}{\min}\underset{D^y}{\max}
    \max_{D^y}
    \; \sum_{e} \alpha_e^y \mathds{E}_{x\sim P(X|Y=y,E)}\log(D^y(F(x))).
     \label{eq:KL_GAN}
\end{equation}
%
We can show it is equivalent to minimize the KL divergence $D_{KL}(P(F(X)|Y)||P(F(X)|Y,E))$.
%
When the number of classes is large, we can use the trick of conditional GAN~\citep{mirza2014conditional} such that all discriminators $D^y, y\in\mathcal{Y}$ can share parameters.
%
In particular, we let the discriminator $D:\mathcal{F}\times\mathcal{Y}\rightarrow [0,1]$ takes both feature representations and the class label as input such that $D^y(F(X)) = D(F(X),y)$.



\noindent\textbf{Model4.}

\noindent\textit{Minimizing Divergence among Conditional Probabilities.} We minimize the divergence among $P(y|\bm{x},e)$, $P(y|\bm{x})$, and  $P(y|\bm{x},e')$, where $e$ is the observed environment and $e'$ is the counterfactual environment.
%
To match the dimension of representation
%
We call this loss model4v1.
%
\begin{equation}
   \mathcal{L}_{model4v1} = \mathcal{L}_{main} + \lambda_1 \sum_{i} D(P(\hat{y}_i|\bm{x}_i)||P(\hat{y}_i|\bm{x}_i,e_i))+\lambda_2 \sum_{i}D(P(\hat{y}_i|\bm{x}_i,e_i)||P(\hat{y}_i|\bm{x}_i,e_i')).
   \label{eq:model4v1}
\end{equation}
In implementation, we consider KL divergence and Wasserstein-1 distance.
%
For the environment variable, we use the mean image in that environment as the input.
%
We use $P(\hat{y}_i|\bm{x}_i,\bar{e})$ as $P(\hat{y}_i|\bm{x}_i)$, where $\bar{e}$ is represented as the mean image of all training images.

\noindent\textit{Minimizing the Gradient against Environment Variables.} We can also impose that the gradient of $P(y|\bm{x},e)$ against the environment $e$ to be zero.
%
This is because we do not want the value of $e$ influences the prediction, given the representation of causal features. Therefore, we formulate the loss function as:
\begin{equation}
    \mathcal{L}_{model4v2} = \mathcal{L}_{main} + \lambda_3 \sum_{i} \left\|\nabla_{e=\hat{e}_i} P(\hat{y}_i|\bm{x}_i,e)\right\|^{2},
\end{equation}
where $\hat{e}_i \in \mathcal{X}$ can theoretically be any image in the input space. This is because we want to make $\left\|\nabla_{e=\hat{e}_i} P(y_i|\bm{x}_i,e)\right\|^{2} \approx 0 $ everywhere.

Then, we also consider a combination of $\mathcal{L}_{model4v1}$ and $\mathcal{L}_{model4v2}$ as $\mathcal{L}_{model4v3}$.

% \noindent\textbf{Data Augmentation.}
%


%

% \noindent\textit{Extrapolation Consistency Training (ECT).} Inspired by Mixup~\citep{zhang2017mixup}, Interpolation Consistency Training (ICT)~\citep{verma2019interpolation} has shown its effectiveness in semi-supervised learning.
% %
% Here, we extend it for out-of-sample generalization.
% %
% We define extrapolation of a pair of instances $(i,j)$ as: \begin{equation}
%     \text{Ext}_{\gamma}(\bm{x}_i,\bm{x}_j) = \gamma \bm{x}_i + (1-\gamma) \bm{x}_j, \gamma\in[-\beta,1+\beta],
% \end{equation} where $\beta>0$ is a hyperparameter.
% %
% Given a pair of instances $(i,j)$, then $f(\text{Ext}(\bm{x}_i,\bm{x}_j))$ should only be correlated with $f(\bm{x}_i)$ and $f(\bm{x}_j)$ and independent of $e_i$ and $e_j$.
% %
% If a pair is from the same class but different environments ($y_i=y_j$ but $e_i\not=e_j$), then we should push $f(\text{Ext}(\bm{x}_i,\bm{x}_j))$ towards predicting $y_i=y_j$ regardless of $e_i$ and $e_j$.
%





% \noindent\textbf{Hierarchical Environments.} Different from the setting of the original IRM paper, in the case of demographics, the environment variable $E$ is often multi-dimensionalvalues and $e=(African, Male, Age > 50)$ and $e'=(African, Male, Age \le 50)$ are both subgroups of African males.
% %
% This motivates us to reconsider how to distinguish the error , the relationships between different environments.
%



% \noindent\textbf{Controlling the Influence of the Environment.}
% %
% According to the causal graph Fig.~\ref{fig:causal_graph2}, we need to control the influence of the environment variable for learning the invariant label prediction function $f$.
% %
% This implies the classifier should model $P(Y|\bm{X},E)$.
% %
% Using deep neural networks, we can instead let the label predicion function $f$ approximate $P(Y|g(\bm{x}),h(\bm{x}))$, where we assume that $\hat{P}(E|h(\bm{x}))$ is an accurate predictor of the environment variable $E$, i.e., the function $h(\bm{x})$ learns representations that are predictive of the environment.
% %
% Thus, we obtain a two-stage training algorithm.
% %
% In the first stage, we learn $h(\bm{x})$ by using the supervision of the environment variable $E$.
% %
% Then, we rely on  $h(\bm{x})$ to control the influence of the environment variable to when we fit the conditional probability $P(Y|g(\bm{x}),h(\bm{x}))$ to make sure we learn invariant representations $g(\bm{x})$ in this case.
% With deterministic $h(\bm{x})$, the invariant predictor $P(Y|g(\bm{x})) = \int P(Y|g(\bm{x}),h(\bm{x}))P(h'(\bm{x})) d h'(\bm{x})  = P(Y|g(\bm{x}),h'(\bm{x}))\mathds{1}(h'(\bm{x})=h(\bm{x}))$.
%


% \noindent\textbf{IRM with Non-dummy Classifiers.} In~\citep{arjovsky2019invariant}, only a dummy classifier $w=1.0$ is considered.
%
% With the dummy classifier $f(g(\bm{x})) = wg(\bm{x}),w=1.0$, $\mathcal{L}_{IRM_{V1}}$ pushes the squared $L_2$ norm of the gradient against $w$ to be $0$ toward satisfying the first order condition~\citep{boyd2004convex}.
% However, in face verification and identification, the deep neural network often consists a backbone representation learner (e.g., ResNet-50) and a head (e.g., softmax).
%
% When the prediction function $f$ is parameterized by a deep neural network, the loss function, in most case, would not be convex w.r.t. the parameters, therefore, we cannot directly apply the $\mathcal{L}_{IRM_{v1}}$ regularizer.
% %

% Recall the original definition of IRM in~\citep{arjovsky2019invariant}, if we train separate label prediction functions for each environment, one heuristic is to enforce $f^e, e=1,...,|\mathcal{E}_{tr}|$ to be similar to each other when training them with by minimizing the cross-entropy error.
% %
% This means we aim to impose $f^e(g(\bm{x})) \approx f^{e'}(g(\bm{x}))$ or  $\hat{P}(Y|g(\bm{x}),e)\approx \hat{P}(Y|g(\bm{x}),e')$.
% %
% When all $f^e$ takes the same family of functions, we only need to enforce their parameters to be similar.
% %
% For example, when $f^e(g(\bm{x}))$ denotes the softmax function and we have $|\mathcal{C}|$ identities in the training data, then we can enforce the weights $\bm{w}_i^e\in\mathds{R}^{d\times 1}, i=1,...,|\mathcal{C}|$ to be similar across environments.
%


% There are two situations. First, we can use separate parameters for each $f^e$.
%
% For those environments not in the training set ($e\in\mathcal{E}\setminus\mathcal{E}_{tr}$), 


